Temporal Tensor Transformation Network for Multivariate Time Series Prediction

Multivariate time series prediction has applications in a wide variety of domains and is considered to be a very challenging task, especially when the variables have correlations and exhibit complex temporal patterns, such as seasonality and trend. Many existing methods suffer from strong statistical assumptions, numerical issues with high dimensionality, manual feature engineering efforts, and scalability. In this work, we present a novel deep learning architecture, known as Temporal Tensor Transformation Network, which transforms the original multivariate time series into a higher order of tensor through the proposed Temporal-Slicing Stack Transformation. This yields a new representation of the original multivariate time series, which enables the convolution kernel to extract complex and non-linear features as well as variable interactional signals from a relatively large temporal region. Experimental results show that Temporal Tensor Transformation Network outperforms several state-of-the-art methods on window-based predictions across various tasks. The proposed architecture also demonstrates robust prediction performance through an extensive sensitivity analysis.

==> sections/5_results.tex <==
\section{Experimental Results}
\input{tables/result.tex}
\begin{figure*}[ht]
    \label{corr_plot}
    \includegraphics[width=\textwidth]{figures/CORR_Plots.png}
    \caption{Empirical Correlation Coefficient Plots by Prediction Horizon}
\end{figure*}

\begin{figure}[ht]
\centering
\includegraphics[width=0.48\textwidth]{figures/prediction_plot.png}
\centering{\caption{Test Prediction Plots}\label{pred_plot}}
\end{figure}

We present the experimental results on the defined metrics presented in Table \ref{results}. For each dataset, we provide the model a fixed input of $T=168$ timesteps and obtained predictions against a horizon window of 15, 30, 60, and 120 timesteps. We note that these horizons are multi-timestep windowed predictions, as opposed to a single-point estimation. The Best performing models with respect to the empirical correlations, are indicated by a bolded font face for each dataset and horizon. We also provide a comparative line graph of the Empirical Correlation Coefficient as shown in Figure \ref{corr_plot}. We also plot sample predictions against our test set, with an empirical comparison against LSTNet, as shown in Figure \ref{pred_plot}.

Based on our empirical results, our proposed model out performs the baseline metrics for Electricity, Solar Energy, and Traffic datasets, while outperforming some of the models for the Exchange Rates dataset. We attribute our analysis based on two key observations: i) the use of stateful versus stateless model types and ii) the autocorrelations present in the dataset.

First, in Figure \ref{corr_plot}, we observe a noticeable cluster between stateless models (i.e. 1D CNN, LSTNet, and TSSNet) and stateful models (i.e. LSTM, GRU, and VAR) in terms of the overall performance. Furthermore, we observe a sharper performance degradation over larger temporal horizon for stateful models than stateless models. Within stateless models, our proposed model consistently retains an upper bound performance, while the 1D CNN model primarily remains as a lower bound with the LSTNet in between. This is also present in the Exchange Rate dataset as well.

The other factor affecting the overall performance of our model is the presence of autocorrelations in the dataset - in particular the seasonality. As previously shown in Figure \ref{acf_plot}, we have noted that there is a strong presence of autocorrelational behaviors found within the Electricity, Solar Energy, and Traffic dataset, while weaker in the Exchange Rate dataset. This realization in context with our empirical results shed light on some observations. For highly autocorrelational data, stateless models tend to perform better over stateful models. However, with weaker autocorrelational signals such as the Exchange Rate dataset, our models perform better than the stateless models, but marginally worse than the stateful model variants.

In particular, our experimental results with 1D CNNs and LSTNet demonstrates that the methods in how convolution is applied over the temporal data can lead to difference in performance. Hence, this provides sufficient evidence that our transformation method enables high efficiency of information gain with respect to the autocorrelational features captured over a large temporal region.
